Faster Lead Optimization Mapper Algorithm for Large-Scale Relative Free Energy Perturbation

In recent years, free energy perturbation (FEP) calculations have garnered increasing attention as tools to support drug discovery. The lead optimization mapper (Lomap) was proposed as an algorithm to calculate the relative free energy between ligands efficiently. However, Lomap requires checking whether each edge in the FEP graph is removable, which necessitates checking the constraints for all edges. Consequently, conventional Lomap requires significant computation time, at least several hours for cases involving hundreds of compounds, and is impractical for cases with more than tens of thousands of edges. In this study, we aimed to reduce the computational cost of Lomap to enable the construction of FEP graphs for hundreds of compounds. We can reduce the overall number of constraint checks required from an amount dependent on the number of edges to one dependent on the number of nodes by using the chunk check process to check the constraints for as many edges as possible simultaneously. Moreover, the output graph is equivalent to that obtained using conventional Lomap, enabling direct replacement of the original Lomap with our method. With our improvement, the execution was tens to hundreds of times faster than that of the original Lomap. https://github.com/ohuelab/FastLomap

==> deepl_en.tex <==

\section{Introduction}

In the early stages of drug discovery, hit-to-lead optimization is used to find lead compounds with sufficient affinity and desirable pharmacological properties from hit compounds that bind relatively weakly to their target receptors.
Alchemical free energy perturbation (FEP) calculations are a powerful tool for lead optimization because perturbation-based methods can calculate the exact relative binding free energies between a candidate compound and its target receptor from molecular dynamics simulations. FEP calculations are a powerful tool to support lead optimization.

In FEP calculations, it is important to provide a closed thermodynamic cycle to correct for errors in the binding free energy calculation.
For closed paths where the total relative free energy is zero, the difference from zero is called the cycle closure error, or hysteresis.
The cycle closure method can improve prediction accuracy over pure perturbation calculations alone by correcting for hysteresis.
Therefore, to guarantee the accuracy of FEP calculations, closed thermodynamic cycles should be added as computational resources permit.
Figure ~\ref{fig:example} shows an example FEP graph of an FEP calculation for the benchmark series of TYK2 targets by Wang et al. run with Cresset Flare's FEP application.

The design-of-experiment problem of how to efficiently perform FEP calculations, taking into account the closed thermodynamic cycle, can be reworded, namely, how the FEP graph, or perturbation map, should be constructed.
First, the most common FEP graph is the star graph. Since it is connected to only one reference compound, it allows FEP calculations with a small number of links, but since there is no single closed thermodynamic cycle, the accuracy of the FEP calculation cannot be guaranteed.
PyAutoFEP provides an implementation that builds wheel-shaped FEP graphs and optimal FEP graphs with Ant Colony Optimization.

Lomap is an automatic algorithm for planning relative free energy calculations.
Lomap provides several design criteria for appropriate relative free energy calculations. Based on the design criteria, a score between compound pairs is calculated and the FEP graph is computed based on the score.
Lomap then constructs the optimal graph based on the criterion that all molecules must be part of at least one closed thermodynamic cycle in constructing the FEP graph.
However, Lomap only generates FEP graphs for a few dozen or so compounds and does not consider the case of hundreds of FEP calculations.

DiffNet~ also provides a theoretical framework for optimizing the covariance matrix with respect to measurement error.
HiMap, developed by the same group as Lomap, also performs statistically optimal design based on optimization of the covariance matrix, similar to DiffNet.

Recently, a machine learning approach called active learning, which is a computer-only design of experiments for lead optimization, has also been attempted for relative coupling free energy calculations.
In active learning, at least hundreds to thousands of large relative coupling free energy calculations are expected.

However, it is difficult to apply the optimal graphs from Lomap directly to active learning, because calculations using conventional Lomap require huge computational costs for FEP graphs for several hundred compounds.
Conventional active learning methods using FEP are limited to either calculating only star-shaped FEP graphs centered on a reference compound or performing more detailed calculations for a limited number of compounds.
Therefore, it is important to be able to easily introduce FEP cycles for hundreds of compounds to support FEP calculations with active learning.

The main reason why the Lomap calculation takes so much time is that the constraint decision is made on the number of edges in the initial graph due to the nature of the algorithm, which determines whether edges can be deleted in a defined order based on certain constraints.
Figure Јref{fig:profile} shows the results of an attempt to generate an FEP graph using the Lomap algorithm for a number of nodes of 1000.
\Most of the time of the function ࿯texttt{build\_graph} is allocated to ࿯texttt{check\_constraints}.

\begin{figure}[tb].
    \centering
    \includegraphics[width=0.8\linewidth]{figure/FEP-graph.pdf}
    \caption{Results of profiles by cProfile of the baseline Lomap algorithm (Thompson TYK2 dataset, $N=1000$). Drawing by snakeviz.}
	\label{fig:profile}
\end{figure}

In this study, we propose a chunk decision process in which edges are processed together as much as possible so that the number of decisions is kept within a constraint that depends on the number of nodes.
The proposed method succeeds in constructing FEP graphs tens to hundreds of times faster than the original Lomap's output FEP graph construction of several hundred compound units.

\section{Methods}
\subsection{Calculation of Link Score}
Lomap comes with an implementation provided based on a freely available API such as RDKit (⌘url{https://github.com/OpenFreeEnergy/Lomap}), which is the main focus of this study.
First, we describe the original Lomap algorithm.
In Lomap, the goal is to create an undirected graph that calculates the relative binding free energy of two compounds.
In order to calculate valid free energies, the FEP graph must consist of edges for sufficiently similar pairs of atoms.
Therefore, a link score is used as a measure of the similarity between two compounds.
The link score is basically calculated based on the maximum common substructure (MCS) between atoms using the following formula.
$S=\exp[-\beta (N_A+N_B-2N_{MCS})]$
where $\beta$ is an arbitrary constant, $N_A$ and $N_B$ are the two input compounds, and $N_{MCS}$ is the number of heavy atoms in the two MCS. That is, the number of insertions and deletions required for the transformation. The score is defined between 0 and 1, with a maximum of 1 when the two compounds are identical.
However, the score is corrected by taking the product of the score calculated based on several other aspects, such as the compounds having the same net charge and preserving the ring as much as possible.
An important point related to our proposal is that edges with low link scores should be preferentially removed as long as they do not affect the FEP graph.
Note that, to construct the FEP graph by the Lomap algorithm, it is necessary to calculate the link scores among all compounds, but since the score calculation for each compound pair can be calculated independently in advance and can be parallelized, the score calculation is not the subject of measurement or acceleration in this study.
\Graph Construction Algorithm with Lomap}
In Lomap, the FEP graph is constructed roughly by the following procedure.
\begin{enumerate}
    \item Calculate the score matrix for all compounds by the score calculation in the previous section.
    \item Generate an initial graph, leaving only edges for pairs whose link scores are above a threshold. The initial graph may be partitioned into multiple subgraphs.
    \item Perform the edge deletion process for each connected component of the initial graph. First, sort the edges in the subgraph in order of decreasing link score. Starting from the edge with the worst link score, we determine whether the constraint is satisfied when the edge is deleted, and if the constraint is satisfied, the edge is deleted; if not, it is left. The four constraints are as follows
    \begin{enumerate}
        The \item subgraph is connected.
	\item The number of nodes not in the cycle does not change (this can be determined by the number of bridges in the cycle not changing)
	\item The diameter of the subgraph is less than or equal to the threshold MAXDIST.
	\item (if necessary) Distance from active known ligand is less than or equal to the threshold.
    \end{enumerate}
    \item Connects subgraphs.
\end{enumerate}
Here, process 3 is the most time-consuming when the graph is huge. This is because 3 determines whether an edge can be deleted or not for every edge in the subgraph each time. And to determine if an edge can be deleted, the process calculates the diameter of the graph and the bridge of the graph. If the number of nodes in the graph is $N$ and the number of edges is $M$, the computational complexity of the diameter is $O(MN)$ and that of the bridges is $O(M+N)$.
The number of edges in the graph changes each time the FEP graph is updated, but with a computational complexity of at least $O(M^2N)$.
The most significant factor of this computational complexity is that for every edge, a decision is made as to whether or not it can be deleted; Lomap deletes edges in order of worst score, and this order must be maintained for consistent constraint judgments. Therefore, the graph generation phase cannot be divided into whole sections and simply computed in parallel.

\Minor modification to the ɑsubsection{diameter calculation}.
The original implementation used networkx's eccentricity method, but the BoundingDiameters algorithm was used.
This is available in the networkx diameter function with the usebounds option.
The diameter calculation is inherently $O(MN)$ computation since it calculates the All Pairs Shortest Path (ASAP).
The algorithm takes advantage of the relationship between the lower and upper bounds between node eccentricity and diameter to perform the exact diameter in a computation time proportional to $O(N)$.
One should be aware of border cases, such as complete graphs and circular graphs~ , but in the case of FEP graph construction, this problem can be ignored.

\subsection{chunk decision process}

This section describes the chunk decision process, which is the core of this study.
In section ref, we mentioned that the constraint decision in Lomap cannot be simply parallelized.
However, since the number of edges in the initial graph is proportional to the square of the number of nodes if no branch and prune is performed, the ratio of edges that do not satisfy constraints follows the inverse of the number of nodes, i.e., the larger the number of nodes, the more edges can be removed for most edges.
Furthermore, the edges that remain due to constraints have the property of being concentrated toward the end of the Lomap algorithm. This is because at the beginning of the procedure, there are many redundant edges, so it is easy to satisfy the constraint by deleting edges, but in the latter part of the procedure, the condition becomes more stringent.
Figure Јref{fig:edges_100} shows the process of deleting edges to generate a FEP graph with 100 nodes. As can be seen from the figure, most of the edges that cannot be deleted are concentrated in the latter half of the process. Therefore, blank areas should be deleted as much as possible at the same time, and edges should be deleted to focus attention on individual edges in areas where non-deletable edges are concentrated.


Given these characteristics of FEP graph optimization, it is likely that the constraint will be satisfied even if many edges are deleted at once in the early stages of the algorithm. Therefore, we propose a chunk constraint decision.

Figure Јref{fig:chunk_check} shows an overview of the chunk decision process.



First, let the chunk scale $S$ be a parameter related to the size of the chunk, and let the chunk level $K$ be the depth of the chunk processing hierarchy, $C_{k}$ being the chunk at chunk level $K$.
Also, for the number of edges $M$, $k_{max}=\lfloor\log_{s}M \rfloor$ represents the maximum chunk level, which means how many times the chunk processing can be done recursively.
The chunk size for the first $k=0$ is $S_0=s^k_{max}$.
For example, when $M=5100$ and $s=10$, $S_0=s^{k_{max}}=10^3$.
The following is the algorithmic procedure for the chunk determination process.
\begin{enumerate}
    \item Perform the constraint check of step (2) for the edges sorted in order of worst link score, $S_0$ from the top.
    \item Constraint check is performed. In the constraint check, the check is considered successful when the constraint is satisfied even if $S_0$ edges are removed. If the constraint is not satisfied (i.e., there are edges in the chunk that cannot be deleted), the check fails and all edges are restored and the next step (3) is performed. If the constraint check succeeds for all edges, return to step (1).
    \item $S_{k}=\max(\lfloor S_{k-1}/s\rfloor , 1)$, perform constraint checks on $S_{k}$ edges of chunk $C_{k-1}$, starting from the top, one by one for $C_k$.
    \item If the edges that cannot be removed are identified, perform constraint checks on the remaining edges of chunk $C_{k-1}$. If the constraint is satisfied, complete chunk processing for chunk $C_{k-1}$ and return to step (2). If not satisfied, continue with step (3) until all edges in the chunk have been successfully checked.
\end{enumerate}

The chunk determination process allows for deletion in large chunk size units in areas where there are few non-deletable edges. In areas with many undeletable edges, individual undeletable edges can be identified without deepening the chunk level. A certain chunk scale is required.

\section{Experiments}
\subsection{Thompson TYK2 dataset}

This time, we will perform FEP experiments with 100 to 1000 nodes for larger FEP graph construction experiments.
Therefore, we used a homogeneous series of TYK2 inhibitors based on aminopyrimidine scaffolds .

\todo{name should be easy to understand}
\begin{description}
    \item[Thompson TYK2 dataset]\mbox{}{}} We randomly selected 1000 cases from the benchmark set and constructed a subset of the experimental set from 100 to 1000 nodes.
    \item[Thompson TYK2$_{0.7}$ dataset]\mbox{}}Complete experimental sets were constructed from the benchmark set with a link score of 0.7 or higher with the reference ligand (4GIH~ ) from 100 to 1000 nodes as well.
\end{description}

Figure Јref{fig:num_edges} shows the number of edges in the two initial graphs relative to the number of nodes for the Thompson TYK2 dataset and the Thompson TYK2$_{0.7}$ dataset.The number of edges in the Thompson TYK2$_{0.7}$ dataset is about 5 times larger than the maximum, and the number of edges is close to the upper limit. The peak of the link score for the Thompson TYK2$_{0.7}$ dataset is higher than the peak of the link score for the Thompson TYK2 dataset. higher than the peak of the link score of the Thompson TYK2 dataset. The number of edges of the optimal graph generated by each number of nodes is shown in Fig.ref{fig:num_edges_opt}. Both methods have the same number of edges in the optimal graph. The generated graphs are equivalent between the proposed and existing methods.

\subsection{Wang-Dataset}
Wang-Dataset is used as a benchmark to evaluate RBFE prediction performance in FEP+ experiments. It is a dataset for eight targets containing about several dozen ligands.
The algorithm proposed in this study assumes that the number of compounds exceeds 100, and its benefit is small under the conditions of such a dataset. Therefore, the Wang-Dataset was used to verify that applying the proposed method in a general use case is not problematic.
The actual ligands used in this experiment are contained in\url{https://github.com/ohuelab/Wang-FEP-dataset}. \모듈을 보보팀 {Because the original is not here, I guess I'll ref the paper and put the dataset at the source publication location as well}.

\subsection{Setup for graph generation}

First, we generate the compound structure for the Thompson TYK2 dataset, since the compound structure is not provided. The compound structures were generated by superimposing on the reference ligand (4GIH~) using the Cresset Flare~ alignment function (⌘texttt{very-permissive} option) for the compounds.

For complex structures, all link score calculations were performed in Lomap's default 3D mode and the pre-computed link scores were used for all experiments. link score calculations for all pairs of 1000 compounds took 26.4 min in parallel processing on 28 CPUs.

Experiments were performed with the original Lomap calculation as baseline and with chunk sizes $s=2, 5, and 10$.

For the generation of the FEP graph, we used the default settings of Lomap: i.e., a graph diameter of 6, no tree structure allowed, and a link score cutoff of 0.4.

\subsection{Results and Disscussion}
\subsection{Results of Thompson TYK2 dataset}
Figure\ref{fig:scale_results} and Figure\ref{fig:scale07_results} show the execution time and number of constraint decisions per number of nodes for the Thompson TYK2 dataset and the Thompson TYK2$_{0.7}$ dataset.
Note that for the cutoff of 0.7, the baseline was after $N=500$ and the calculation was not completed in 24 hours.
For the Thompson TYK2$_{0.7}$ dataset, the maximum is about 23.7 times faster when the number of nodes is 1000.
And in the case of the Thompson TYK2$_{0.7}$ dataset, it is several hundred times faster when the number of nodes is 400, and the baseline method cannot construct the FEP graph when $N=500$ or more. As explained in the previous section, the number of edges in the SIMILAR dataset increases due to the low effectiveness of branch pruning, and the baseline method, which performs the number of constraint decisions by the number of edges, cannot handle it. Thus, the proposed method is effective when the number of edges is extremely large.

\subsection{Results of Wang-Dataset}
Figures ≪ref{fig:benchmark_results} and ≪ref{fig:scale07_results} show the execution time and number of constraint decisions for each number of nodes in the Wang-dataset.
The larger the number of nodes, the longer the execution time tends to be, but it is only slightly shorter than baseline at $s=5, 10$. The proposed method is also faster than the baseline method, but within 3 seconds at the most. Therefore, we can say that the proposed method has no negative impact on the conventional use cases.
\싉TODO{If we could also compare profiles (but not in the PDPTA submission version)}

\section{Conclusion}

In order to promote the use of relative binding free energy calculations in drug discovery, we have modified the Lomap algorithm to be scalable to an increasing number of compounds.
While the proposed method is not effective for the conventional use of a few dozen compounds in general, it enables a speedup of several tens of times or more for several hundred cases. The output graph of the proposed method is equivalent to that of the original Lomap algorithm, so it can be used immediately in that it can replace existing methods without modification.

Although not addressed in this study, speeding up the link score calculation is also an issue for future work.
If the link score is calculated for all compound pairs, the amount of calculation increases by an order of magnitude of two.
In Himap, unsupervised clustering using the DBSCAN method is used to group compounds by similarity. The amount of computation may be reduced by clustering by a faster method such as compound fingerprinting, and then performing score calculation based on common substructures.
In addition, the graph generation stage is not important because it may take several minutes to calculate link scores for all compound pairs in conventional graph generation of several dozen cases.
Therefore, it is necessary to devise a way to skip the calculation of compound pairs with link scores lower than a certain level in advance.

Then, it is debatable whether the Lomap algorithm is appropriate for large-scale designs.
The recently published Himap method extends the Lomap algorithm and adds discussions on the number of nodes and the accuracy of the perturbation map.
It is important to elucidate to analyze the impact of cycle closure redundancy on the accuracy of perturbation maps in large FEP graphs.

The proposed method efficiently identifies the necessary edges for the optimal graph from an initial graph with hundreds of thousands of edges, allowing the calculation of relative coupled free energy with cycle closure even for 1000 cases.
By utilizing the proposed method, it is not just a matter of planning FEP experiments for large FEPs, but also an application to active learning methods for relative coupled free energy calculations.

